Federated Learning with Only Positive Labels by Exploring Label Correlations

Federated learning aims to collaboratively learn a model by using the data from multiple users under privacy constraints. In this paper, we study the multi-label classification problem under the federated learning setting, where trivial solution and extremely poor performance may be obtained, especially when only positive data w.r.t. a single class label are provided for each client. This issue can be addressed by adding a specially designed regularizer on the server-side. Although effective sometimes, the label correlations are simply ignored and thus sub-optimal performance may be obtained. Besides, it is expensive and unsafe to exchange user's private embeddings between server and clients frequently, especially when training model in the contrastive way. To remedy these drawbacks, we propose a novel and generic method termed Federated Averaging by exploring Label Correlations (FedALC). Specifically, FedALC estimates the label correlations in the class embedding learning for different label pairs and utilizes it to improve the model training. To further improve the safety and also reduce the communication overhead, we propose a variant to learn fixed class embedding for each client, so that the server and clients only need to exchange class embeddings once. Extensive experiments on multiple popular datasets demonstrate that our FedALC can significantly outperform existing counterparts.

==> text/abstract-V1.tex <==
\begin{abstract}

Federated multiple Label learning aims to complete multi-label classification tasks by collaboratively training machine (deep) learning models under privacy constraints, facing the problem of the collapse of the model and thus resulting
in trivial solution or extremely poor performance. To cope with it, most of existing works adopt the coarse regularizer on the server-side, especially in the scenario of federated learning with only positive label. Though effective, they ignore label correlations in multi-label space and simply treat each label as equal. In this work, we propose a novel and generic method termed Federated Averaging by exploring Label Correlations methods, dubbed FedALC, to bridge this gap in federated multiple label learning. Specifically, to address the lack of correlations, FedALC calculates label correlation weights in the class embedding learning for different label pairs and utilizes it to improve the quality of the training process. To improve the safety and reduce the communication overhead, we also propose a variant to learn fixed class embedding for each corresponding client, so that the server and client only need to exchange class embeddings once. Extensive experiments on multiple popular datasets demonstrate that our FedALC can significantly outperform existing counterparts.

\end{abstract}
\begin{IEEEkeywords}
Federated learning, machine learning, multi-label classification.
\end{IEEEkeywords}




==> text/conclusion-V1.tex <==
\section{Conclusion and Discussion}
\label{sec:Conclusion}

In this paper, we investigate the problem of the multi-label classification in the federated learning setting, where each client has only access to the local dataset associated with positive data, and propose a novel method that explores the label correlations to improve the quality of the class embedding matrix. Existing algorithm treats different labels equally, while our FedALC can explore label correlations by making the best of the distribution of labels. To improve safety and reduce the computational cost and communication overhead, we further propose a variant of our FedALC by learning a fixed class embedding matrix, where the server and clients only need to exchange class embeddings once. Moreover, a sophisticated strategy is designed for label collection. The experiments show that our algorithm is more adaptive and effective for federated multi-label classification.

In regard to limitations, simply using positive class embedding to replace the corresponding instance embedding may lead to information loss, especially in the variant of learning fixed class embedding. Exploring how to find better surrogate for instance embedding may further improve the performance and also accelerate the learning process. Besides, we mainly conduct experiments on multi-label datasets with limited communication rounds and relatively small or moderate number of class labels, and the effectiveness on more massive-scale extreme multi-label datasets should be verified. Addressing these limitations will be left as our future work.

==> text/experiments-V1.tex <==
\section{Experiments}
\label{sec:Experiments}

We empirically evaluate the proposed FedALC method on diverse multi-label dataset, including both the popular visual and very challenging text datasets. We use cosine similarity to define the distance, i.e.,
\begin{equation}
{d}_{\cos }\left({x}, {y}\right)=1-{x}^{\top}{y}, \quad \forall{x},{y}\in \mathbb{R}^{d}.
\end{equation}
Given the specific distance function, the positive loss in the client can be given as follow:
\begin{equation}\label{postive loss}
    \ell_{cl}^{\mathrm{pos}}(\mathbf{x},y)={\max}({0, 0.9-g_{\theta}({\mathbf{x}})^{T} \mathbf{w}_{y}})^{2}.
\end{equation}
In our experiment, we follow the setting of positive loss in \cite{yu2020federated} that encourages all pairs of positive instance and its label $(x,y)$ to have dot product larger than $0.9$ in the embedding space. 


\begin{table}[!t]
    \caption{A summary of the datasets used in multi-label image classification experiments.}
\centering
    \begin{tabular}{@{}lccccc@{}}    
        \toprule          
         %最上面的横线
        {\scriptsize\textbf{Dataset}} &{\scriptsize\textbf{Labels}} &  {\scriptsize\textbf{Training images}} & {\scriptsize\textbf{Validation images}}& {\scriptsize\textbf{Test images}} \\ 
        \midrule
        COCO&80&73,873&8,208&4,0136\\
        
        VOC12&20&10,963&577&5,823\\
        
        VOC07&20&4,761&250&4,952\\
        \bottomrule
    \end{tabular}
    \label{iamge_data_table}
\end{table}

\subsection{Datasets}
We use three benchmark datasets for multi-label image classiﬁcation, i.e., COCO\cite{lin2014microsoft}, VOC 2012\cite{everingham2010pascal} and VOC 2007\cite{everingham2010pascal}. A summary of three datasets is presented in Table~\ref{iamge_data_table}.
The hyper-parameters in our compared experiments are all same. The \textbf{COCO} dataset contains a total of 122,218 images associated with 80 labels. We use the original training set and randomly select $10\%$ as Validation. The original Validation set is used for testing. The VOC 2012 (\textbf{VOC12}) dataset contains a total of 17,363 images associated with 20 labels. The original training set contains 11,540 images for training and Validation. Because of the small number of the datasets, we just randomly select $5\%$ as Validation and the rest for training. The original Validation set containing 5,823 is used for testing. The VOC 2007 (\textbf{VOC07}) dataset contains a total of 9,963 images associated with 20 labels. The original training set contains 5,011 images for training and Validation. we do the same as the VOC12 experiment and just randomly select $5\%$ as Validation and the rest for training. The original Validation set containing 4,952 is used for testing.

\begin{table}[!t]      
%h：hear，t：top，b：bottom，p：page，下一页。
\caption{Summary of the dataset: N is the number of training instances, M is the number of test instances. F is the total features, L is the total umber of class labels. I/L is the number of instances per label, and L/I is the number of labels per instance}
\centering
\label{tab1}
\setlength{\tabcolsep}{3mm}
    \begin{tabular}{@{}lcccccc@{}}    
    %几列就写几个c，表示内容居中写，哪里需要分割线就在哪里加“|”
        \toprule           
         %最上面的横线
        {}&{N} & {M} & {F}& {L}& {I/L}& {L/I} \\ 
        \midrule
        EURLex&15539&3809&5000&3993&25.73&5.31\\
        
        Bibtex&4880&2515&1836&159&111.71&2.40\\
        \bottomrule
    \end{tabular}
\label{text_inf}
\end{table}
We also evaluate our algorithm on extreme multi-label text datasets: EURLex\cite{Menca2008EfficientPM} and Bibtex\cite{2008Multilabel}. These datasets are available in the Extreme Classification Repository\footnote{Most of the popular extreme classification datasets are available on the website:http://manikvarma.org/downloads/ XC/XMLRepository.html}. A statistic of the sample, feature and class label of EURLex and Bibtex are shown in Table~\ref{text_inf}.

\subsection{Model architecture}
As mentioned earlier, we use a simple embedding-based classification model. For image datasets, we use \textbf{RESNET-50} \cite{he2016deep} as the backbone. The feature is then mapped into $512$-dimensional vector using linear transformation. Finally, the embedding is normalized so that its $l_2$-norm is $1$. For text datasets, high-dimensional sparse vector is embedded into $\mathbb{R}^{512}$ by embedding layer. The output is then passed through three linear layers with the size of $1024$, $1024$ and $512$. The first two layers use a ${ReLU}$ activation function. The output is then normalized to the unit vector. The instance embedding and class embedding are all $l_2$ normalized, and thus the predicted score belongs to the $[-1,1]$ interval.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth,scale=1.00]{acc_big.pdf}
    \caption{A comparison of our FedALC and the FedAwS counterpart under different hyper-parameter settings Precision@1,3,5($\%$) with K=5 on the EURlex dataset.}
    \label{fig:Accuracy on Eurlex}
\end{figure*}
\subsection{Implementation detail}
The methods are implemented using PyTorch, and all experiments are performed on server containing CPUs of 2.60GHz and GPUs of GeForce RTX 3090. SGD (stochastic gradient descent) is used to optimize the embedding-based model. We follow the setting in~\cite{yu2020federated} to use a large learning rate ($0.1$) when optimizing the instance embeddings on the clients, to accelerate the learning process. The learning rate on the server is set as $0.0001$. Most of the hyper-parameters in our FedALC method are the same as FedAwS, in which the balancing hyper-parameter $\lambda$ is tuned to achieve the best performance. Figure \ref{fig:client_len} is a statistic of the number of instances for all labels (clients) on the EURlex dataset, where we can see that the numbers vary significantly for different labels, and exhibit a long-tail distribution, this distribution is also existing in other datasets in our experiments. In the following experiments, we let all clients  participate in the communication to accelerate the training process. For image datasets, we run $100$ global communication rounds on COCO and $300$ rounds on VOC12 and VOC07. For text datasets, we limit global communication rounds in the experiment of dynamic class embedding to $300$ and $500$ rounds for the fixed embedding variant.

\subsection{Compared baselines}
To show the effectiveness of the proposed method, we compare the proposed method with the following approaches:
\begin{itemize}
\item{\textbf{SLEEC\cite{bhatia2015sparse}:}} Training by employing SLEEC in the oracle mode, which has access to both positive and negative embeddings. \item{\textbf{FedAvg\cite{mcmahan2017communication}:}} Training by employing FedAvg with only positive loss. In order to reduce the possibility of the collapse as much as possible, we initialize the class embedding matrix that is almost spreadout.
\item{\textbf{FedAwS}\cite{yu2020federated}:} Training by employing FedAwS with stochastic negative mining and the balancing hyper-parameter $\lambda$ controlling the effect of the spreadout on the class embedding matrix.
\item{\textbf{FedAvg-fixed:}} Training by employing FedAvg with only positive loss with the fixed class embedding, which is generated by random.
\end{itemize}

\subsection{Evaluation criteria}
For multi-label classification datasets, especially text datasets, even though the label space is very large, each instance only has several relevant labels. Hence, it is crucial to choose the short and most relevant label list for each test instance and evaluate the prediction quality, where the label list is the short ranked list of potentially relevant labels. The classic evaluation metric for the multi-label text classification is the top $K$ precision ($P@K$). We use this metric to evaluate the quality of the prediction with $K=1,3,5$. We denote $y\in \{ 0, 1 \}^{L}$ as the vector of true labels of an instance, and $\hat{y}\in R^{L}$ as the algorithm-predicted score for the instance. Then the metric can be defined as :
\begin{equation}
    P@K=\frac{1}{k} \sum \limits_{l\in r_{k}(\hat{y})} y_{l}
\end{equation}
where $r_{k}(\hat{y})$ is the set of rank indices of the truly relevant labels among the top-$k$ portion of the algorithm-predicted ranked list for an instance. In multi-label image classification, we use classic mean average precision~(MAP)\cite{wang2020multi} and also $P@K$ as the evaluations criteria.

\begin{table}[!t]
%h：hear，t：top，b：bottom，p：page，下一页。
\caption{MAP($\%$) and Top-k($\%$) on multi-label image datasets.}
\centering
\label{tab1}
\setlength{\tabcolsep}{5mm}
    \begin{tabular}{@{}l|ccc@{}}    
         \toprule       
         %最上面的横线
        {Dataset}&{Method}&{MAP}&{P@3} \\ 
        \hline  
        \multirow{5}{*}{COCO} &FedAwS&30.33&\textbf{25.72}\\
       
        ~&\textbf{FedALC~(Our)}&\textbf{30.35}&25.60\\
      
        \cline{2-4}
        ~&FedAvg-fixed&26.86&20.26\\
       
        ~&\textbf{FedALC-fixed~(Our)}&\textbf{30.22}&\textbf{25.03}\\
         \hline  
        \multirow{5}{*}{VOC12} &FedAwS&37.70&18.04\\
     
        ~&\textbf{FedALC~(Our)}&\textbf{40.78}&\textbf{20.41}\\
       
         \cline{2-4}
   
        ~&FedAvg-fixed&37.19&17.40\\
       
        ~&\textbf{FedALC-fixed(Our)}&\textbf{43.33}&\textbf{22.77}\\
        \hline  
        \multirow{5}{*}{VOC07} &FedAwS&41.65&21.16\\
  
        ~&\textbf{FedALC~(Our)}&\textbf{42.73}&\textbf{23.00}\\
   
        \cline{2-4}
     
        ~&FedAvg-fixed&41.54&21.56\\
      
        ~&\textbf{FedALC-fixed~(Our)}&\textbf{42.66}&\textbf{21.56}\\
        \bottomrule
    \end{tabular}
\label{result_image}
\end{table}

\subsection{Experiments on multi-label image datasets}
The results are shown in Table \ref{result_image}.
From the table, we can see that: 1) since the number of labels is not very large for these datasets, the superiority of FedAwS compared with FedAvg is limited. This may be because the numbers of labels are not very large in these datasets, and it is easy to initialize a dispersed class embedding matrix, which is similar to one obtained by simple spreadout, as adopted in FedAwS. By exploring label correlations, our FedALC consistently outperforms FedAvg under different criteria; 2) our method consistently outperforms FedAwS in terms of MAP, and is superior to FedAwS in most cases on $P@3$. In particular, we achieve a significant $8.17\%$ relative improvement in terms of MAP on VOC12.
we also find that the performance on fixed class embeddings is better than the dynamic one in the experiment of VOC12. The reasons behind this are that: 1) the high-quality fixed class embedding which is spreadout enough and contains label correlations may achieve satisfactory performance; 2) the number of labels is so limited in the multi-label images datasets where the number of classes is often lower than 100, compared with the thousands in the text datasets. In this case, class embeddings have enough space(i.e. 512-dimensional space in this case) and is easy to achieve high quality, so that may results in better results. Regarding the dynamic embeddings, the optimizations of class embeddings in client and server are aimed to draw them close and disperse them, which are contradictory operations and may get stuck in training process.
\subsection{Experiments on multi-label text datasets}
\begin{figure}[!t]
    \begin{center}
      \includegraphics[width=\linewidth]{all_acc.pdf} 
    \end{center}
    \caption{P@1($\%$)on Eurlex.}
    \label{fig:P@1 on Eurlex}
\end{figure}

\begin{figure}[!t]
    \begin{center}
      \includegraphics[width=\linewidth]{client_len.pdf} 
    \end{center}
    \caption{Visualization of number heterogeneity among users on EURlex dataset.}
    \label{fig:client_len}
\end{figure}

 The results on Bibtex are shown in Table \ref{Bibtex_result} and Figure \ref{fig:EURlex_Bibtex_fixed_C}(a), and the results on EURlex are reported in Table \ref{Eurlex_result} and Figure \ref{fig:EURlex_Bibtex_fixed_C}(b). In particular, the learning curves of our FedALC and FedAwS under different $\lambda$ in terms of $P@1$ on the Eurlex dataset are shown in Figure \ref{fig:P@1 on Eurlex}. The corresponding results in terms of precisions at different $k$ are shown in Figure \ref{fig:Accuracy on Eurlex}.

From the results, we can see that: 1) the FedAvg algorithm prematurely converged and lead to relatively low accuracy because of the collapse; 2) the proposed FedALC is much better than FedAvg in learning either dynamic or fixed class embeddings since our correlations regularizer well handles with the problem of collapse ; 3) FedAwS is quite sensitive to the hyper-parameter $\lambda$. When the value of $\lambda$ is too small, the class embeddings cannot be well separated and this leads to collapsing issue and thus low accuracy. When $\lambda$ is too large, the class embedding matrix is over spreadout. The instance embedding is hard to approach corresponding positive class embeddings, and hence the performance may also be poor; 4) Our FedALC can balance the dispersion and closeness of positive embeddings to some degree by exploring label correlations and automatically setting the weights for different label pairs. In particular, we achieve a significant $19.3\%$ relative improvement in terms of $P@1$ on the Bibtex dataset. FedALC disperses the matrix by taking label correlations into consideration, highly-correlated classes would be closer than those in FedAwS, and thus instance embedding would be easier to get close to its positive class embeddings and results in more similarity. In regard to FedAwS utilizing stochastic negative mining, the given label and most of the selected neighbors are correlated with each other. Simply making them be arbitrary spreadout is thus sub-optimal. Whereas in our FedALC, more attention is paid on dispersing the embeddings of uncorrelated labels, and hence better performance can be obtained. This further verifies the beneﬁt of exploring the label correlations.

\begin{table}[t]      
%h：hear，t：top，b：bottom，p：page，下一页。
\caption{Precision@1,3,5($\%$) with K=5 on EURlex.}
\centering
\label{tab1}

\setlength{\tabcolsep}{5mm}
    \begin{tabular}{@{}l|cccc@{}}  
        \toprule           
        {Method}&{$\lambda$}&{P@1}&{P@3}&{P@5} \\ 
        \hline
         {SLEEC~(Oracle)}&{}&{{63.40}}&{{50.35}}&{{41.28}}\\
         {FedAvg}&{}&{29.61}&{21.85}&{17.95}\\
        \hline
        \multicolumn{5}{c}{$\mathbf{K=5}$}\\
        \hline
        \multirow{6}{*}{FedAwS}&{1}&{43.10}&{31.32}&{24.57}\\
       
         {}&{10}&{49.80}&{35.93}&{28.05}\\
       
         {}&{100}&{46.96}&{33.71}&{26.78}\\
      
         {}&{150}&{48.01}&{36.77}&{29.91}\\
    
         {}&{200}&{47.25}&{35.78}&{29.01}\\
  
         {}&{500}&{31.08}&{21.41}&{17.22}\\
         
         \hline
         {\textbf{FedALC~(Our)}}&{1}&{\textbf{54.02}}&{\textbf{38.72}}&{\textbf{31.04}}\\
         \bottomrule
    \end{tabular}
\label{Eurlex_result}
\end{table}

\begin{table}[!t]      
%h：hear，t：top，b：bottom，p：page，下一页。
\caption{Precision@1,3,5($\%$) with K=5 on Bibtex.}
\centering
\label{tab1}
\setlength{\tabcolsep}{5mm}
    \begin{tabular}{@{}l|cccc@{}}    
        \toprule          
        {Method}&{$\lambda$}&{P@1}&{P@3}&{P@5} \\ 
        \hline
        {SLEEC~(Oracle)}&{}&{{65.08}}&{{39.64}}&{{28.87}}\\
         {FedAvg}&{}&{11.6}&{9.11}&{7.84}\\
         \hline
         \multicolumn{5}{c}{$\mathbf{K=5}$}\\
        \hline
         \multirow{6}{*}{FedAwS}&{1}&{16.42}&{11.91}&{10.45}\\
       
        &{10}&{26.79}&{18.05}&{14.58}\\
      
         {}&{100}&{48.31}&{30.85}&{23.66}\\
       
         {}&{150}&{48.42}&{30.78}&{23.43}\\
       
          {}&{200}&{49.22}&{30.74}&{23.11}\\
      
         {}&{500}&{45.65}&{28.09}&{21.43}\\
         \hline
         {\textbf{FedALC~(Our)}}&{1}&{\textbf{58.72}}&{\textbf{35.83}}&{\textbf{26.62}}\\
         \bottomrule
    \end{tabular}
\label{Bibtex_result}
\end{table}

\begin{figure}[!t]
    \begin{center}
      \includegraphics[width=\linewidth]{fixed.pdf}
    \end{center}
    \caption{Performance~($P@k$) comparison of FedALC-fixed and FedAvg-fixed, FedAvg on Bibtex and EURlex.}
    \label{fig:EURlex_Bibtex_fixed_C}
\end{figure}


==> text/introduction-V1.tex <==
\section{Introduction}
Federated learning (FL)~\cite{mcmahan2017communication} is a novel machine learning paradigm that trains an algorithm across multiple decentralized clients (such as edge devices) or servers without exchanging local data samples. Since clients can only access the local datasets, the user's privacy can be well protected, and this paradigm has attracted increasing attention in recent years~\cite{li2020federated}.
In this paper, we study the challenge problem of learning a multi-label classification model~\cite{liu2017deep} under the federated learning setting, where each user has only local positive data related to a single class label~\cite{yu2020federated}. This setting can be treated as the extremely label-skew case in the data  heterogeneity of federated learning, which is popular in real-world applications. For example, a user verification (UV) model is decentralized and cooperatively trained by aggregating sensitive information of multiple users, and each client has only access to specific information (such as voice~\cite{2017Deep}, face~\cite{2018Additive}, fingerprint\cite{Cao2019Automated} and iris\cite{nguyen2017iris}) of a single user.

The key challenges for federated learning with only positive labels is the collapse of the model. In our setting, each client lacks negative information including negative instances and negative class embeddings. Hence, naively employing vanilla federated learning algorithms such as Federated Averaging (FedAvg) and especially considering embedding-based model~\cite{vaswani2017attention, konevcny2016federated}, may cause the collapse of class embeddings and result in a trivial solution or extremely poor performance~\cite{bojanowski2017unsupervised}, since the client neglects the negative loss and only indiscriminately minimizes the distance between positive instance embedding and the class embedding. In this case, different class scores on a test sample will be similar and indistinguishable, resulting in the meaningless trained model.
%\ls{reorganize this paragraph. it seems that the first three sentences is not related to only positive learning! }


This issue is investigated and initially addressed by a recent work \cite{yu2020federated}, where an algorithm termed Federated Averaging with Spreadout (FedAwS) is proposed by imposing a geometric regularization on the server-side to separate different class embeddings and prevent them collapsing to a single point.
This approach, however, treats different labels equally in the spreadout (class embedding separation) process. That is, embeddings of class labels that are highly correlated and significantly different in multiple labels space are separated in the same way. This is not reasonable since embeddings should be close for correlated labels, and dissimilar otherwise. For example, we assume that the class labels 'Desktop computer’ and ’Desk’ often appear in the same instance, thus these two corresponding class
embedding vectors can be deemed high-correlation and may be relatively close compared with others, such as class labels 'aircraft', 'automobile', etc. Besides, since the instance and class embeddings are trained on clients and server respectively, the class embeddings should be transmitted frequently between the server and clients. Privacy leakage may occur in the transmission process, and the leakage risk would increase significantly with an increasing number of transmissions.
\ls{The drawbacks and limitations of current solution. (The motivation of our work)}

\begin{figure*}[t]   
    \begin{center}      
    \includegraphics[width=2\columnwidth]{FedALC_Overview-V2.pdf}    
    \end{center}
    \caption{\textbf{Algorithm Overview}. The \textbf{FedALC} algorithm \textbf{(1)} computes gradients and hash code locally. The instance hash code is utilized for calculating label correlations and \textbf{only need transmission once}, we will illustrate it in the later section. The client then sends \textbf{(2)} model parameters, class embedding, and hash code to the server. On the server, \textbf{(3)} The global model is obtained via aggregation and \textbf{(4)} the class embedding matrix, and label distributions are obtained by incorporation. \textbf{(5)} The server then utilizes our core correlation regularizer to optimize the class embedding matrix and obtains the trained class embedding matrix, \textbf{(6)}and eventually transmits global model parameters and corresponding class embedding to the client.}
    \label{pipeline}
\end{figure*}


Observing the challenge in the collapse of model and the limitations of prior art, we propose a novel method termed Federated Averaging by exploring Label Correlations, named FedALC (see Figure \ref{pipeline}), for FL with only positive labels. In particular, to address the lack of labels correlations, we construct a novel regularizer to optimize the class embedding matrix by taking the label correlations into consideration. This is achieved by adding a correlation-based weight for each label pair in the spreadout, so that embeddings of similar labels are relatively close and dissimilar labels are far away. In this case, the label correlation can be well considered meanwhile the problem of collapse can be addressed. Besides, to reduce both the computational cost and transmission overhead, we propose a variant to learn fixed class embedding matrix so that only a single transmission of class embeddings between the server and clients should be conducted. To implement the label correlation regularizer performed on the server, we also propose an encrypted transmission strategy to collect label information across clients and obtain label distributions on the server. The label distributions are then utilized for calculating the weight of the correlation between different labels.

To summarize, the main contributions of this paper are:
\begin{itemize}
  \item We propose a novel method termed FedALC to exploit the correlations between different class labels for federated learning with only positive labels. Our method can make the embeddings of relevant labels close to each other and stay away from irrelevant labels in class embedding learning;
  \item We propose a variant that learns fixed class embeddings to improve safety and reduce transmission overhead.
  \item We design an encrypted and communication-efficiency strategy for calculating label correlations by collecting labels across clients and constructing label distributions on the server;
\end{itemize}
We conduct extensive experiments on three popular visual datasets and two challenging multi-label text datasets. The results demonstrate significant improvements over the competitive counterparts. For example, we achieve relative improvements of $8.17\%$ and $19.3\%$ on the VOC 2012~\cite{everingham2010pascal} and Bibtex~\cite{2008Multilabel} datasets respectively compared with FedAwS.

The rest of paper is organized as follows. In section 2, we review related work about multi-label learning and federated learning. Section 3 introduced the problem of multi-label federated learning with only positive labels. Section 4 presents the FedACL algorithm in detail. In section 5, we show experiments on multi-label datasets and results. Section 6 summarizes this paper.



==> text/methodology-V1.tex <==
\section{Federated Averaging by Exploring Label Correlations}
\label{sec:Method_FedALC}

%\ls{overall pipeline of FedALC. FedALC is composed of XXX, XXX and XXX. Highlevel benefits of each components.}
In this section, we proposed Federated Averaging by exploring Label Correlations (FedALC) which employs a two-stage strategy. The first stage is the optimization of the client with the local loss (Eq.\ref{client_loss}). Then clients transmit model parameters and class embedding to the server. The classic operation of averaging is done on the model parameters with no extra processing step. The second stage is the core of our contribution that is the optimization of class embedding matrix with the proposed label correlations regularizer, this stage is performed on the server. To assist in completing the calculation of label correlations between multiple labels, we also proposed the encrypted and communication efficiency method to collect label information across clients in FL setting. Two variances of label correlations regularizer and the method of collection are depicted as following:

\subsection{Spreadout by exploring label correlations}
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=\columnwidth]{FL.png}
    \end{center}
    \caption{Mechanism of the designed correlation regularizer under the centralized and federated paradigm. The red, blue and green dots indicate the instance, positive class and negative class respectively.}
    \label{fig:Norm_Fed_Contrast}
\end{figure}
To exploit label correlations, we need to first collect the label set for each instance. This process will be explained later. Given the collected label sets, we propose to add a correlation regularizer on the server-side to improve the dispersion of class embedding matrix by taking the label correlations into consideration. We first define $L_{j}^{P}$ and $L_{j}^{N}$ as the positive and negative label set for the $j$-th instance, respectively. For example, in a five-class classification problem, there is an instance with labels $\{0,1,2\}$, and then its label set is $L_{j}=[L_j^{P},L_j^{N}]$, where the positive label set $L_{j}^{P}=[0,1,2]$ and negative label set $L_{j}^{N}=[3,4]$. We collect the label sets of all clients' instances and merge them on the server, and the resulting whole label set is: ${L}=\{(L_{1}^{P},L_{1}^{N}),(L_{2}^{P},L_{2}^{N}),...,(L_{n_\mathrm{all}}^{P},L_{n_\mathrm{all}}^{N})\}$, where $n_\mathrm{all}$ is number of all clients' instances. Then the correlation regularizer can be given as follow:

\begin{equation}
\label{eq:corr_reg}
\begin{split}
&\operatorname{reg}_{\mathrm{cr}}(W)
=\sum_{i \in[m]}\frac{|\mathcal{S}^{i}|}{|\mathcal{S}|} \hat{\mathcal{R}}_{\mathrm{neg}}\left(\mathcal{S}^{i}\right)\\
&\!=\!\!  \frac{1}{n_{all}}\sum\limits_{i\in [m]}\sum\limits_{j\in [n_{i}]}\ell^{\mathrm{neg}}_{cl}({L_{j}^{P}}, {L_{j}^{N}},W)\!\!\\
&\!=\!\! \frac{1}{n_{all}} \sum\limits_{j\in [n_\mathrm{all}]}\!\! \left( \frac{1}{|L_{j}^{P}|}\sum\limits_{y_j \in L_{j}^{P},\atop y_j^{\prime} \in L_{j}^{N}}\! \left(\max \left\{0, \nu \!-\!d(\mathbf{w}_{y_j}, \mathbf{w}_{y_j^{\prime}})\right\}\right)^{2}\right)\\
&\!=\!\!\sum_{u \in[C]}\!\! \left(\sigma_{uu'}\cdot \sum_{u^{\prime} \neq u}
\left(\max \left(0, \nu\!-\!d(\mathbf{w}_{u}, \mathbf{w}_{u^{\prime}})\right)\right)^{2} \right),
\end{split}
\end{equation}
where $\sigma_{uu'}$ is a weight that reflects the correlations of different class labels. The weight is larger for more dissimilar labels and thus the dispersion would focus more on these labels. Since the number of instances for different labels may vary significantly, we add a normalization term to balance different labels, i.e.,
\begin{equation}
\begin{split}
\operatorname{reg}_{\mathrm{cr}}(W)
&\!=\!\!\sum_{u \in[C]}\!\left(\gamma_{uu'} \sum_{u^{\prime} \neq u}\left(\max\{0, \nu\!-\!d\left(\mathbf{w}_{u}, \mathbf{w}_{u^{\prime}}\right)\}\right)^{2} \right),
\end{split}
\end{equation}
where $\gamma_{uu'} = \frac{\sigma_{uu'}}{\sum_{u^{\prime} \neq u} {\sigma_{uu'}}}$.
To avoid the exhaustive tuning of hyper-parameter $\nu$, we follow~\cite{reddi2019stochastic, yu2020federated} to reformulate (\ref{eq:corr_reg}) as:
\begin{equation}
\begin{split}
\operatorname{reg}_{\mathrm{cr}}^{\mathrm{top}}(W)
&\!=\!\!\sum_{u \in[C]}\!\! \left(\sigma_{uu'} \sum_{u^{\prime} \neq u,\atop u^{\prime} \in \mathcal{N}_{\mathcal{K}}(u) }
\left(\max \left(0, \nu\!-\!d(\mathbf{w}_{u}, \mathbf{w}_{u^{\prime}})\right)\right)^{2} \right)
\end{split}
\end{equation}

where $\mathcal{K}$ is the number of a subset of classes, and $\mathcal{N}_{k}(u)$ is the set of $\mathcal{K}$ classes that are most close to the class $u$ in the embedding space. we can also normalize the weight of correlations $\sigma_{uu'}$ to obtain $\gamma_{uu'}$ in this case. From the instance viewpoint, our correlation regularizer regards the set of positive class embeddings as the surrogate of its instance embedding in the client negative loss of Eq.~(\ref{client_loss_expected}). Hence, the surrogate negative loss doesn't need instance embeddings and only needs class embeddings, which can be accessed in the server. According to the class embedding matrix and collected label sets, the surrogate negative losses of all clients can be jointly calculated on the server-side. Figure~\ref{fig:Norm_Fed_Contrast} illustrates the mechanism of our correlation regularizer under the centralized and federated paradigms. Under the centralized paradigm, the instance is enforced to be close to positive class embeddings, and separated from negative class embeddings. Under the federated paradigm, in the client optimization, the local steps presented in Fig.\ref{pipeline}  enforce the instance embedding to be close to positive class embeddings. On the server side, the correlation regularizer makes the positive and negative class embeddings stay away from each other.

\subsection{Learning fixed class embedding}
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=1\columnwidth]{fixed_class_embedding.png}
    \end{center}
    \caption{FedALC with a fixed class embedding matrix. On the server side, positive class embeddings are enforced to be close and separated from negative class embeddings. Then the fixed class embeddings are obtained; On the client side, the instance are enforced to approach its positive classes.}
    \label{fixed_class_embedding}
\end{figure}

In the above approach, the class embeddings are transmitted frequently between the server and clients. This may lead to the occurrence of privacy leakage, since the class embedding contains the identity information of users, especially when dealing with the face recognition task. To remedy this drawback and reduce the overhead, we propose a variant of our method to learn fixed class embeddings so that the transmission of class embeddings is performed only once. Since we want the class embedding matrix to be fixed and cannot be updated alternatively, the learned embedding matrix should be of high quality. This is achieved by using the positive class embedding to replace the corresponding instance embedding in both terms of Eq.(\ref{client_loss_expected}) to learn a fixed class embedding matrix. According to the distribution of label sets, we define the correlation regularizer for learning the fixed class embedding matrix as follows:
\begin{equation}\label{fixed_reg}
\begin{split}
&\mathrm{reg}_{\mathrm{fc}}(W)
=\sum_{i \in[m]}\frac{|\mathcal{S}^{i}|}{|\mathcal{S}|}\left((\hat{\mathcal{R}}_{\mathrm{pos}}\left(\mathcal{S}^{i}\right)+\hat{\mathcal{R}}_{\mathrm{neg}}\left(\mathcal{S}^{i}\right)\right)\\
&= \frac{1}{n_{all}}\sum\limits_{i\in [m]}\sum\limits_{j\in [n_{i}]}\left(\ell^{\mathrm{pos}}_{cl}({L_{j}^{P}}, {L_{j}^{N}},W)+\ell^{\mathrm{neg}}_{cl}({L_{j}^{P}}, {L_{j}^{N}},W)\right)\\
&=\frac{1}{n_{all}} \sum\limits_{j\in [n_\mathrm{all}]} \left( \frac{\alpha}{|L_{j}^{P}|}\sum\limits_{y_j \in L_{j}^{P},\atop y_j^{\prime} \in L_{j}^{P} \And  y_j^{\prime}\neq y_{j}} \left(d(\mathbf{w}_{y_j}, \mathbf{w}_{y_j^{\prime}})\right)^{2} \right.\\ 
&\left.+\frac{\beta}{|L_{j}^{P}|}\sum\limits_{y_j \in L_{j}^{P},\atop y_j^{\prime} \in L_{j}^{N}}\left(\max \left\{0, \nu -d(\mathbf{w}_{y_j}, \mathbf{w}_{y_j^{\prime}})\right\}\right)^{2}\right)
\end{split}
\end{equation}

For each instance, the positive loss in Eq.(\ref{fixed_reg}) encourages the positive embedding to be close and the negative loss in it encourages negative and positive embedding to be far away from each other. This process is illustrated in Figure \ref{fixed_class_embedding}, where the server learns a fixed class embedding matrix using regularizer Eq.(\ref{fixed_reg}) and sends it to each clients. In the client optimization, the local step makes the instance embedding approach its positive class embeddings. The transmission of fixed class embeddings between clients and the server is only needed  once since the obtained class embeddings are unchanged during the process of federated learning.


\subsection{Label sets collection}
There still remains a question on how to collect the labels for each instance. In multi-label classification, an instance may have multiple labels. Since each client is associated with a single label, the same instance may be distributed in different clients. To collect the labels for each instance, we propose to first use the irreversible hash algorithm, such as MD5~\cite{rivest1992md5} or SHA~\cite{wang2005finding} and all other Message Digest algorithms~\cite{bellovin2005deploying,coron2005merkle}, to map the instance embedding into the low-dimensional hash vector on the client side. Here, we assume that embeddings of the same instance on different clients are the same (i.e., the same feature extractor is adopted). Then the hash messages together with the associated labels are sent to the server. Finally, the received messages are compared and labels of the same messages are merged to obtain the label sets. The main procedure is illustrated in Figure~\ref{collect label}, where we transmit the hash messages instead of the original instance embeddings since: 1) instance embedding contains the user's identity information, and it is unsafe to exchange them between the server and clients. Some techniques (such as GAN) can be adopted to recover the user's data \cite{Sun_2021_CVPR}; 2) the embedding may be of large size and thus incur a large communication overhead.

\begin{figure}[t]
    \begin{center}
      \includegraphics[width=\linewidth]{collect.png}  
    \end{center}
    \caption{Label sets collection for each instance in the federated setting. Embeddings of the same data point on different clients are mapped as hash messages, which are sent to the server together with the label information. Then the server compare the messages and aggregate the labels that have the same message.}
    \label{collect label}
\end{figure}

In Algorithm~\ref{alg}, we summarize the learning procedure of FedALC method. We separate the label collection part and the learning part in a light of clarity. Actually, the label collection can be performed together with the class embedding updates at the first round of communication.

\begin{algorithm}[!t]
	\caption{Federated Averaging by exploring Label Correlations (FedALC) with collecting label sets} 
	\label{alg} 
	\begin{algorithmic}[1]
		\STATE \textbf{Input:} $m$ clients, $\mathcal{S}^{i}$ at the $i$-th client.
		\STATE Server initializes parameters $\theta^{0}$, embeddings $W^{0}$, hashing function $H$.
		\STATE Server sends the initialization to clients.
		\STATE \textbf{Collecting label sets:}
		\STATE \textbf{for} i=1,2,3,...,m \textbf{do}:
		\STATE \quad The $i$-$th$ client downloads the initialization.
		\STATE \quad Compute hash vectors on the local data set:\\ \quad $M_{i}\gets H(g_{\theta}(\mathcal{S}^{i})) $
		\STATE \quad The $i$-th client sends the $M_{i}$  to the server.
		\STATE \textbf{end for}
	    \STATE Server integrates the $M_{i}$: $L \gets
	    \mathrm{merge}(M_{i})$
	    \STATE \textbf{Federated learning process:}
	    \STATE \textbf{for} t=0,1,2,...,T-1 \textbf{do}:
	    \STATE \quad Server sends $\theta^{t}$, $W^{t}$ to the $i$-th client
	    \STATE \quad \textbf{for} i=1,2,...,C \textbf{do}
	    \STATE \quad \quad $\left(\theta^{t}_{i}, \mathbf{w}^{t}_{y_{i}}\right) \leftarrow\left(\theta^{t}_{i}, \mathbf{w}^{t}_{y_{i}}\right)-\eta \nabla_{\left(\theta^{t}, \mathbf{w}^{t}_{y_{i}}\right)} \hat{\mathcal{R}}_{\text {pos }}\left(\mathcal{S}^{i}\right)$
	    \STATE \quad \quad $\text{where } \hat{\mathcal{R}}_{\text {pos }}\left(\mathcal{S}^{i}\right)=\frac{1}{n_{i}} \sum_{j \in\left[n_{i}\right]} \ell_{\mathrm{cl}}^{\mathrm{pos}}(\mathbf{x}^{i}_{j}, w^{t}_{y_i}).$
	    \STATE \quad \quad 
	    The $i$-th client sends $(\theta^{t}_{i}, \mathbf{w}^{t}_{y_{i}})$ to the server.
	    \STATE \quad \textbf{end for}
	    \STATE \quad Server updates the model parameters by averaging :\\
	    \quad $\theta ^{t+1}=\frac{1}{C} \sum\limits_{i\in [C] }\theta^{t}_{i}$,
	    \STATE \quad Server merges the class embedding and gets $W^{t}$
	    \STATE \quad$ W^{t+1} \leftarrow \tilde{W}^{t+1}- \lambda \eta \nabla_{\tilde{W}^{t+1}} \operatorname{reg}_{\mathrm{c}}\left(\tilde{W}^{t+1}\right)$.
	    \STATE \textbf{end for}
	    \STATE \textbf{Output:} $\theta^{\mathrm{opt}},W^{\mathrm{opt}}$.
	\end{algorithmic} 
\end{algorithm}

\subsection{Discussion with FedAwS}
Based on the FedAvg framework~\cite{mcmahan2017communication}, a recent work termed Federated Averaging with Spreadout (FedAwS)~\cite{yu2020federated} is presented to handle this federated multiple labels setting that clients have only access to the positive data for a single class. To address the challenge of this issue, the FedAwS framework uses a spreadout strategy to optimize the class embedding matrix, which can disperse the embedding matrix and arrest the trend of collapse. This is achieved by letting the server perform an geometric regularizer to ensure that class embeddings are separated from each other, in addition to averaging shared model parameters.

This process can be formulated as applying the following geometric regularization in each communication round on the server:
\begin{equation}
\operatorname{reg}_{\mathrm{sp}}(W)=\sum_{u \in[K]} \sum_{u^{\prime} \neq u}\left(\max \left(0, \nu-d\left(\mathbf{w}_{u}, \mathbf{w}_{u^{\prime}}\right)\right)\right)^{2},
\end{equation}
where $K$ is the number of classes. Since the hyper-parameter $\nu$ may be very hard to choose, FedAwS also reformulate (3) as:
\begin{equation}
\operatorname{reg}_{\mathrm{sp}}^{\mathrm{top}}(W)=\sum_{u\in [K]}\sum_{u' \in \mathcal{K}', \atop u' \neq u}-d^{2}\left(\mathbf{w}_{u}, \mathbf{w}_{u'}\right) \cdot \llbracket u' \in \mathcal{N}_{k}(u) \rrbracket,
\end{equation}
where $\mathcal{K}'$ is a subset of classes, and $\mathcal{N}_{k}(u)$ is the set of $k$ classes that are close to the class $u$ in the embedding space. This is motivated by the stochastic negative mining approach~\cite{reddi2019stochastic}. Since only the distances between close class embeddings are maximized, the computational cost can be reduced. 

A main drawback of FedAwS is that the embeddings of different classes are separated in the same way without considering the correlations between different class labels as mentioned above. The simple spreadout regularizer is effective in the task of multi-class classification but may be coarse in multiple labels task due to the lack of label correlations. Motivated by the above discovery, we mainly tackle this issue by exploring label correlations.



==> text/problem_setup-V1.tex <==
\section{Problem Formulation}
\label{sec:Problem_Formulation}

We consider the embedding-based model~\cite{vaswani2017attention, konevcny2016federated} to complete multi-label classification task under the federated learning setting, where each client has only access to the local dataset associated with a single label. We suppose that there are $m$ clients, and the $i$-th client is associated with a single label $y^{i}$. In multi-label classification, an instance may have multiple labels, and hence the same instance may be distributed in different clients. For $i \in [m]$, the ${i}$-th client has access to the local dataset $\mathcal{S}^{i}=\{(\mathbf{x}_{1}^{i},y^{i}),(\mathbf{x}_{2}^{i},y^{i}),\cdots,(\mathbf{x}_{n_{i}}^{i},y^{i})\} $. An embedding network $g_{\theta}: \chi \rightarrow \mathbb{R}^D$ maps the input $\mathbf{x}$ as the $D$-dimensional instance embedding $g_{\theta}(\mathbf{x})$. The label of all $n_{i}$ instances are the same since each client only has a single label.
Given a distance measure $d(\cdot,\cdot)$, the contrastive loss~\cite{oord2018representation} used in clients can be given by:
\begin{equation}
\begin{split}
\ell_{\mathrm{cl}}(\mathbf{x}_j^{i},y^{i},\theta,W)=\alpha \cdot\left(d\left(g_{\boldsymbol{\theta}}(\mathbf{x}_j^{i}), \mathbf{w}_{y^{i}}\right)\right)^{2} +\quad \quad \quad\quad \quad\\
\quad \quad \quad \beta \cdot \sum_{c \neq i}\left(\max \left\{0, \nu-d\left(g_{\boldsymbol{\theta}}(\mathbf{x}_j^{i}), \mathbf{w}_{y^{c}}\right)\right\}\right)^{2}\quad,
\end{split}
\label{client_loss_expected}
\end{equation}
where $\alpha$ and $\beta$ are trade-off hyper-parameters, $\theta$ is parameters of model(feature extractor), $W \in \mathbb{R}^{C \times D}$ is the class embedding matrix ($C=m$ in our single label setting) and $D$ is the dimension of embedding, with each row being a class embedding $\mathbf{w}_{y^{c}}$. The front and back item of Eq.\ref{client_loss_expected} is termed positive loss and negative loss, respectively. Then, the prediction function can be expressed as:
\begin{equation}
    f(\mathbf{x})=W g_{\boldsymbol{\theta}}(\mathbf{x}).
\end{equation}
Since the client has no access to the instances of negative classes in our setting, we rewrite the loss function (Eq.\ref{client_loss}) as the following form by dropping the negative loss:
\begin{equation}
\ell^{\mathrm{pos}}_{cl}(\mathbf{x}_j^{i}, \mathbf{w}_{y^{i}})=d^{2}\left(g_{\boldsymbol{\theta}}(\mathbf{x}_j^{i}), \mathbf{w}_{y^{i}}\right).
\label{client_loss}
\end{equation}
Then the empirical loss on the local dataset $\mathcal{S}^{i}$ can be given by:

\begin{equation}
\hat{\mathcal{R}}_{\mathrm{pos}}\left(\mathcal{S}^{i};\mathbf{w}_{y^{i}}\right):=\frac{1}{n_{i}} \sum_{j \in\left[n_{i}\right]} \ell^{\mathrm{pos}}_{cl}\left(\mathbf{x}_j^{i}, \theta, \mathbf{w}_{y^{i}}\right).
\end{equation}

To avoid the collapse of class embedding matrix in our setting, we adopt the classic strategy that adds a geometric regularizer to let the matrix be spreadout, and the optimization of the whole objective function is given as follows:
\begin{equation}
\begin{split}
&\qquad\qquad\qquad \quad \min \limits_{\theta, W} \mathcal{L}(\theta,W,\mathcal{S}),\\
&\operatorname{where} {\mathcal{L}}:= \sum_{i \in[m]}\frac{|\mathcal{S}^{i}|}{|\mathcal{S}|} \hat{\mathcal{R}}_{\mathrm{pos}}\left(\mathcal{S}^{i}\mathbf{;{w_{y_{i}}}}\right)+\lambda \cdot \mathrm{reg}_{\mathrm{sp}}(W).\\
%&=\frac{1}{|\mathcal{S}|} \sum_{i \in[m]} \sum_{j \in\left[n_{i}\right]} \ell^{\mathrm{pos}}_{cl}\left(\mathbf{x}_j^{i}, \theta, \mathbf{w}_{y^{i}}\right)+\lambda \cdot \mathrm{reg}_{\mathrm{sp}}(W).
\end{split}
\end{equation}

The objective is to minimize both the sum of each client's empirical risk and the structure risk of class embedding matrix, and $\lambda$ is the balancing parameter. The former term encourages instance embeddings $g_{\boldsymbol{\theta}}(\mathbf{x}^{i})$ to be close to the corresponding class embedding $\mathbf{w}_{y^{i}}$, which is performed on the client. The latter disperses the class embedding matrix, which is performed on the server. 

\ls{please give the optimization model}


==> text/related_work-V1.tex <==
\section{Related Work}
\label{sec:Related_Work}

\subsection{Multi-label learning}
We first introduced Multi-class learning before Multi-label learning. Multi-class learning is the problem of classifying instances into one of multiple classes. In contrast to the traditional classification problem where only a single class label is assigned to an instance~\cite{wang2018baseline,tsoumakas2009mining,zhang2013review}, a single instance may have more than one label in multi-label classification (MLC), which can be utilized in a variety of applications ranging from protein function classification~\cite{barutcuoglu2006hierarchical}, document classification~\cite{yang2016hierarchical}, to automatic image classification~\cite{wang2016cnn}. A dozen of works have proposed various settings of MLC with limited supervision. For example, partial multi-label~(PML)~\cite{xie2018partial} studies a problem that a superset of labels is given. Multi-label learning with missing labels (MLML)~\cite{sun2010multi} assumes that only a subset of labels is obtained. A thorough review of multi-label methods can be found in~\cite{liu2021emerging}.
Besides, in this era of big data, the extreme multi-label learning~(XMLC)~\cite{jain2016extreme} with a large number of labels has attracted more and more attention and becomes a new mainstream direction of MLC. 

\subsection{Federated learning}
Federated learning~(FL) is a distributed machine learning paradigm that multiple clients collaborate to complete a learning task without exchanging privacy data, while maintaining communication efficiency. A well-known and commonly used FL algorithm is Federated Averaging~(FedAvg)\cite{mcmahan2017communication}, which learns a global model by simple averaging.
Recently, numerous and more sophisticated algorithms or aggregation strategies have been proposed to address various FL challenges. For example, the performance of local models may be better than the global model due to the distribution divergence issue, and personalized federated learning~\cite{2021Exploiting,2021Personalized,2020Ditto} was proposed to address this issue by adopting a personalized method to optimize the global model for each client.
In~\cite{2012Privacy,mcmahan2017communication,2019Federated}, some new approaches are designed for better privacy protection, while other works \cite{2020Acceleration,2020Qsparse} mainly focused on reducing communication cost. More recent works assume a heterogeneous setup that data on different clients hold different distributions~\cite{2021Data,2021Bias,2020KD3A}. Client clustering and selection are also studied~\cite{2021Heterogeneity,2021Clustered,2020An}. In this paper, we study a challenging FL setting that each client has only access to positive data following~\cite{yu2020federated}.

The most related work to our proposed FedALC is FedAwS \cite{yu2020federated}. However, our work is different from the former work by the following considerations: \textbf{1)} our approach constructs the correlation regularizer from the perspectives of instances but FedAwS consider the class to construct its class-spreadout regularizer; \textbf{2)} To improve safety and reduce communication overhead, we also extend our approach to a variant where learn fixed class embedding for each client, and thus client and server only need transmit class embedding once; \textbf{3)} To accomplish our correlation regularizer in the server, we also propose a novel strategy to collect label correlations across clients with the guarantee of safety and communication efficiency. 
%\ls{State the difference (1)(2)(3)(4)}

